Continuous Deep Learning: A Workflow to Bring Models into Production

Researchers have been highly active to investigate the classical machine learning workflow and integrate best practices from the software engineering lifecycle. However, deep learning exhibits deviations that are not yet covered in this conceptual development process. This includes the requirement of dedicated hardware, dispensable feature engineering, extensive hyperparameter optimization, large-scale data management, and model compression to reduce size and inference latency. Individual problems of deep learning are under thorough examination, and numerous concepts and implementations have gained traction. Unfortunately, the complete end-to-end development process still remains unspecified. In this paper, we define a detailed deep learning workflow that incorporates the aforementioned characteristics on the baseline of the classical machine learning workflow. We further transferred the conceptual idea into practice by building a prototypic deep learning system using some of the latest technologies on the market. To examine the feasibility of the workflow, two use cases are applied to the prototype.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

In this paper, we described a detailed step-by-step \ac{dl} workflow, split into three pipelines, such that each component is independently reproducible and thereby enabling fast iterations.
These pipelines in turn can further include sequences of automated steps.
For example, the data management pipelines constructed in \cref{subsubsec:data_pipeline_implementation} include separated downstream pipelines for preparing data and storing labels, respectively.
Together with additional pipelines for \ac{ci}/ac{cd}, a project team can quickly face the challenge of \enquote{pipeline jungles} introduced by Sculley \etal~\cite{sculley_hidden_2015}.
Managing these pipelines thus requires frequent knowledge exchange, versioning, and well-connected interfaces.

Considering our abstraction of the \ac{dl} workflow derived in \cref{sec:workflow}, it becomes apparent that there is a dependency on various persistence entities with different functions.
This increases data management costs and complicates collaboration, as knowledge about storing and retrieving data is required.
On the contrary, these \entityNeutral{persistence entities} are required to keep the workflow reproducible.
With continuous iterations of the \ac{dl} lifecycle, it becomes important to align the related data between \entityNeutral{persistence entities}.
As an example, additional effort is required to keep the registered model and the version in the \entityNeutral{Code Repository} aligned.
From a technical perspective, both the \entityNeutral{Model Registry} and \entityNeutral{Code Repository}, are crucial.
On the one hand, \acp{vcs} do not allow storing large artifacts such as a \ac{dl} model.
On the other hand, a \entityNeutral{Model Registry} cannot provide a history of code changes, and efficiently hold all source code of the \ac{dl} workflow.
An adopted \ac{vcs} concept that manages \ac{ml} data, model artifacts, workflow source code, etc., as a single set of dependencies in a central location would facilitate the \ac{dl}, and the \ac{ml} workflow in general.
There are certain tools such as \textit{DVC} and \textit{CML}~\cite{iterative} that focus on this concept.
However, these are incompatible with the requirements of the \ac{dl} workflow since they do not provide scalability and compute resource orchestration.

Through a prototype, we showed that it is possible to translate the conceptual idea to practice using the latest technologies available on the market.
It becomes clear that a large amount of different technologies is necessary to execute the complete \ac{dl} lifecycle.
Although there are all-in-one solutions available, these technologies often suffer from vendor lock-in and are associated with high costs, and they are not directly targetted towards \ac{dl}.
The large technology stack imposes the need for interfaces between tools, activities, and roles.
This in turn introduces additional hazards to the implemented workflow.
Taking \stepDataLabeler{Data Labeling} as an example: we use \pach since it allows building scalable data pipelines, and managing compute resources.
As \pach does not provide any labeling features, \textit{Label Studio} is introduced.
To store our labels to a \textit{PostgreSQL} table, \pach again facilitates export and import.
Thus, we use a complex constellation of technologies within the data pipeline, which can become confusing and error-prone.

Through the application of two distinguished use cases, we demonstrated the practicability of our workflow.
However, the use cases do not represent the complexity of real-world challenges.
For example, we worked with exemplary datasets that do not require sophisticated data pipelines.
Additionally, because our models in production are not exposed to actual requests, we did not implement \stepDataScientist{Model Monitoring} in our prototype.
Thus, we cannot tackle problems such as concept drift.
Therefore, further evaluation is required to investigate the validity of the presented \ac{dl} workflow, and extend the prototype with the not yet implemented steps.
Furthermore, we restricted our investigation to supervised \ac{dl}.
However, unsupervised approaches may exhibit a deviating development workflow and reveal limitations.


==> tables/workflow_technologies.tex <==
\rowcolors{2}{gray!10}{}
\begin{tabular}{
    lll
}

\hiderowcolors
\toprule

\textbf{Technology} & \textbf{Purpose} & \textbf{Persistence Entity} \\

\midrule
\showrowcolors

GitLab~\cite{GitLabInc.2021} & Version control, \ac{ci}/\ac{cd} & Code Repository \\
MinIO~\cite{MinIOInc2021} & Object storage & Model Registry \\
PostgreSQL~\cite{PostgreSQLGlobalDevelopmentGroup2021}  & Store labels and experiment data & ML Data \\
Label Studio~\cite{HeartexInc.2021} & Data labelling & -- \\
Pachyderm~\cite{PachydermInc.2021} & Data lineage, object storage & ML Data, Transformation Registry \\
Determined~\cite{DeterminedAI2021} & Model pipeline & Model Registry \\
Seldon~\cite{SeldonTechnologiesLtd2021} & Model deployment & -- \\

\bottomrule

\end{tabular}

